The Hypervolume Indicator: Problems and Algorithms

The hypervolume indicator is one of the most used set-quality indicators for the assessment of stochastic multiobjective optimizers, as well as for selection in evolutionary multiobjective optimization algorithms. Its theoretical properties justify its wide acceptance, particularly the strict monotonicity with respect to set dominance which is still unique of hypervolume-based indicators. This paper discusses the computation of hypervolume-related problems, highlighting the relations between them, providing an overview of the paradigms and techniques used, a description of the main algorithms for each problem, and a rundown of the fastest algorithms regarding asymptotic complexity and runtime. By providing a complete overview of the computational problems associated to the hypervolume indicator, this paper serves as the starting point for the development of new algorithms, and supports users in the identification of the most appropriate implementations available for each problem.

==> preamble.tex <==
% \citestyle{acmnumeric}
\setcitestyle{numbers,sort&compress}


\usepackage{setspace}
% \usepackage[usenames,dvipsnames]{xcolor}
\usepackage[utf8]{inputenc}
\usepackage{graphicx}
\usepackage{multirow}
\usepackage{tabularx}
\usepackage{placeins}
\usepackage{xfrac}
% 
\RequirePackage{subfigure}
% 
\usepackage[normalem]{ulem} 
\usepackage{fancyhdr}
\usepackage{epigraph}
\usepackage{todonotes}
\usepackage{bm}

% For algorithms
\usepackage{algorithm}
\usepackage[noend]{algorithmic}
\renewcommand{\algorithmiccomment}[1]{$/\!/$ #1}

\newcommand{\mymultiline}[1]{
\begin{tabular}{c}
#1
\end{tabular}}

%left aligned
\newcommand{\mymultilinel}[1]{
\begin{tabular}{l}
#1
\end{tabular}}

% \usetikzlibrary{bayesnet}
\usepackage{microtype}

% para ter footnotes nas tabelas
\usepackage{footnote}
\makesavenoteenv{tabular}

\setlength\tabcolsep{1.5pt}

\newcommand{\specialcell}[2][c]{%
\begin{tabular}[#1]{@{}c@{}}#2\end{tabular}}



\definecolor{mydarkblue}{rgb}{0,0.08,0.45}
\definecolor{cool_blue}{RGB}{48,127,175}

% \usepackage{hyperref}
% \hypersetup{
% %     colorlinks,
% %     citecolor=mydarkblue,
%     citecolor=black,
%     %citecolor=black,
%     filecolor=black,
%     linkcolor=black,
%     urlcolor=mydarkblue,
% %     pdfauthor={\thesisauthorb},
% %     pdftitle={\thesisttlb}
% }
% \usepackage{natbib} % AG - deixei comentado, se descomentar as citacoes passam a ter nome e ano


\usepackage{graphicx}
\usepackage{listings}
\usepackage{nomencl}

\usepackage{etoolbox}

\RequirePackage{subfigure}
\usepackage{amsmath,amssymb}
\usepackage{amsthm}
\usepackage{boxedminipage}
\usepackage{rotating}
\usepackage{enumerate}

\setcounter{tocdepth}{2}
\usepackage{url}
\usepackage{xspace}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{lscape}
\usepackage{array}
\usepackage{mdwlist}

\usepackage{xcolor}
\usepackage{placeins}

\usepackage[percent]{overpic}

\usepackage{sidecap}
\usepackage{wrapfig}

\usepackage{grfext}


\usepackage[portuguese,english]{babel}
\addto{\captionsenglish}{\renewcommand{\bibname}{References}}


% ----------------- Coloured text/comments ------------------------------ %

\usepackage{comment}

\newcommand\myworries[1]{\textcolor{red}{#1}}
\newcommand\hide[1]{}
\newcommand\agchange[1]{\textcolor{orange}{#1}}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\renewcommand\agchange[1]{\textcolor{black}{#1}}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


% --------------------------------------------------------- %
% ----------------- Counters ------------------------------ %

%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \newcounter{paraa}[section]
\newcounter{paraa}% New counter pagecntr is reset with an increment in chapter

% \newcounter{para}[subsection]
\newcounter{para}[section]
\newcounter{sssi}[subsubsection]
% \newcommand\myparagraph[1]{\par\medskip\refstepcounter{para}\textbf{[\Alph{paraa}\arabic{para}]}\space\textbf{#1}\newline}
\newcommand\myparagraph[1]{\par\medskip\refstepcounter{para}\textbf{[\Alph{paraa}\arabic{para}]}\space\textbf{#1}.\ }
\newcommand\myparref{\refstepcounter{para}[\Alph{paraa}\arabic{para}]}
\renewcommand{\thepara}{[\Alph{paraa}\arabic{para}]}
% thepara
% \renewcommand{\thesubsection}{\refstepcounter{paraa}\thechapter.\thesection.\thesubsection}


% --------------------------------------------------------- %



%preferir pdfs antes de pngs, svg,...
\AtBeginDocument{%
  \PrependGraphicsExtensions*{
    .mps,.MPS,.pdf,.PDF,.eps,.EPS,.ps,.PS,
    .png,.PNG,.jpg,.jpeg,.JPG,.JPEG,
    .funny,.foobar
  }%
  \PrintGraphicsExtensions % see .log file
}


\newcommand{\procedure}[1]{\textsf{#1}}
% \newcommand{\argmin}{\ensuremath{\procedure{argmin}}}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\maximize}{maximize}
\DeclareMathOperator*{\minimize}{minimize}
\DeclareMathOperator*{\st}{subject\:to}
% \DeclareMathOperator*{\min}{min}


\newcommand{\ie}{i.e.}% id est  --       that is
\newcommand{\eg}{e.g.}% exempli gratia -- for example
\newcommand{\etal}{\emph{et al.}}% et alii -- and others
\newcommand{\wlogg}{w.l.o.g.}% exempli gratia -- for example
\newcommand{\wrt}{w.r.t.~}% exempli gratia -- for example


\newcommand{\X}{\mathcal{X}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Xr}{\mathrm{X}}
\newcommand{\Ir}{\mathrm{I}}
\newcommand{\Irs}{\mathrm{I^\smile}}
\newcommand{\Irf}{\mathrm{I^\frown}}
\newcommand{\Ell}{\mathrm{L}}
\newcommand{\J}{\mathrm{J}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Sr}{\mathrm{S}}
\newcommand{\Srg}{\Sr^\textrm{g}}
\newcommand{\Sropt}{\Sr^\textrm{opt}}
\newcommand{\Jr}{\mathrm{J}}
\newcommand{\Rr}{\mathrm{R}}
\newcommand{\Prm}{\mathrm{P}}
\newcommand{\Qr}{\mathrm{Q}}
\newcommand{\Tr}{\mathrm{T}}
\newcommand{\Ar}{\mathrm{A}}
\newcommand{\Lr}{\mathrm{L}}
\newcommand{\Br}{\mathrm{B}}
\newcommand{\Cr}{\mathrm{C}}
\newcommand{\Ps}{\mathrm{P}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\Rn}{\mathbb{R}^n}
\newcommand{\Rnn}{\mathbb{R}^{n\times n}}
\newcommand{\Rd}{\mathbb{R}^d}
\newcommand{\Rm}{\mathbb{R}^m}
\newcommand{\Rtwo}{\mathbb{R}^2}
\newcommand{\Rt}{\mathbb{R}^3}
\newcommand{\Rf}{\mathbb{R}^4}
\newcommand{\indicator}{{\bf I}}
\newcommand{\cx}[1]{\ensuremath{{#1}_{x}}}
\newcommand{\cy}[1]{\ensuremath{{#1}_{y}}}
\newcommand{\cz}[1]{\ensuremath{{#1}_{z}}}
\newcommand{\cw}[1]{\ensuremath{{#1}_{w}}}
\newcommand{\cd}[2]{\ensuremath{{#1}_{#2}}}
\newcommand{\ndd}{\ensuremath{\procedure{nondominated}}}
\newcommand{\ssp}{\ensuremath{\procedure{subsetSelection}}}



% -------------------------- HV Problems ----------------------------------%

\newcommand{\hvp}{\textsc{Hypervolume}}
\newcommand{\allcp}{\textsc{AllContributions}}
\newcommand{\allcps}{\textsc{AllContributions2}}
\newcommand{\onecp}{\textsc{OneContribution}}
\newcommand{\setcp}{\textsc{SetContribution}}
\newcommand{\mincrp}{\textsc{LeastContributor}}
\newcommand{\hvupdp}{\textsc{UpdateHypervolume}}
\newcommand{\allcupdp}{\textsc{UpdateAllContributions}}
\newcommand{\allcupdps}{\textsc{UpdateAllContributions2}}
\newcommand{\hssp}{\textsc{HSSP}}
\newcommand{\hsspc}{\textsc{HSSPComplement}}



\newcommand{\NPhard}{\ensuremath{\mathcal{NP}}-hard\xspace}
\newcommand{\mcol}{\multicolumn}
\newcommand{\cmnt}[1]{\noindent {\bf[ #1 ]}}

\newcommand{\lexlt}{\mathrel{<_L}}

\newcommand{\x}[1]{\ensuremath{{#1}_{x}}}
\newcommand{\y}[1]{\ensuremath{{#1}_{y}}}
\newcommand{\z}[1]{\ensuremath{{#1}_{z}}}
\newcommand{\w}[1]{\ensuremath{{#1}_{w}}}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand{\Ctr}{H}

% Logical operators (not to mix 'join' with 'or')
\newcommand{\orl}{\mbox{ \textbf{or} }}
\newcommand{\andl}{\mbox{ \textbf{and} }}

% Among vectors
\newcommand{\nondom}{\parallel}
\newcommand{\weakdom}{\leq}
\newcommand{\dom}{\prec}
\newcommand{\ndominates}{\nprec}
\newcommand{\strictdom}{<}
\newcommand{\strongdom}{\ll}
% Among sets
\newcommand{\Weakdom} { \preceq } 
\newcommand{\Elemwisedom}{ \mathrel{\prec\!\!\cdot} }
\newcommand{\Strictdom} { \prec }
\newcommand{\Strongdom} { \pprec }
% $\preceq$, $\lhd$, $\prec$ or $\pprec$

\newcommand\pprec{\prec\mkern-5mu\prec}


\graphicspath{
    {images/}{images/hssp/}
    {images/hssp/gHSS2DColours/}
    {images/hv-stoa/}{images/hv-stoa/2D/}{images/hv-stoa/3D/}{images/hv-stoa/3D/DefsNProblems/}
    {results/figuresTEC-HVC/}    
    }
    


% ----------------------------------------------------
% \theoremheaderfont{\normalfont\bfseries}

\newtheoremstyle{mystylet}% name
  {\topsep}% Space above               %\topsep
  {\topsep}% Space below               %\topsep
  {\itshape}% Body font                 %\normalfont
  {0pt}% Indent amount
  {\bfseries}% Theorem head font
  {.}%Punctuation after theorem head
  {5pt plus 1pt minus 1pt}%Space after theorem head
  {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}% theorem head spec
\theoremstyle{mystylet}


\newtheorem{theorem}{Theorem}[section]
\newtheorem{lemma}[theorem]{Lemma}
\newtheorem{proposition}[theorem]{Proposition}
\newtheorem{corollary}[theorem]{Corollary}
\newtheorem{conjecture}[theorem]{Conjecture}



\renewenvironment{proof}[1][Proof.]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\qed\end{trivlist}}
\newenvironment{example}[1][Example]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}
\newenvironment{remark}[1][Remark]{\begin{trivlist}
\item[\hskip \labelsep {\bfseries #1}]}{\end{trivlist}}

\newtheoremstyle{mystyle}% name
  {\topsep}% Space above               %\topsep
  {\topsep}% Space below               %\topsep
  {\normalfont}% Body font                 %\normalfont
  {0pt}% Indent amount
  {\bfseries}% Theorem head font
  {.}%Punctuation after theorem head
  {5pt plus 1pt minus 1pt}%Space after theorem head
  {\thmname{#1}\thmnumber{ #2}\thmnote{ (#3)}}% theorem head spec
\theoremstyle{mystyle}


\newtheorem{definition}{Definition}
%
\newtheorem{problem}{Problem}

% 
% \makeatletter
% \AfterEndEnvironment{definition}{\noindent}
% \makeatother
% %        
% 
% \widowpenalty=0
% \clubpenalty=0
% \brokenpenalty=0

